Pioneer Agent: Continual Improvement of Small Language Models in Production

Small language models are attractive for production deployment due to their low cost, fast inference, and ease of specialization. However, adapting them to a specific task remains a challenging engineering loop, driven not by training itself but by surrounding decisions: data curation, failure diagnosis, regression avoidance, and iteration control. We present Pioneer Agent, a closed-loop system that automates this lifecycle. In cold-start mode, given only a natural-language task description, the agent acquires data, constructs evaluation sets, and iteratively trains models by jointly optimizing data, hyperparameters, and learning strategy. In production mode, given a deployed model with labeled failures, it diagnoses error patterns, constructs targeted training data, and retrains under explicit regression constraints. To evaluate this setting, we introduce AdaptFT-Bench, a benchmark of synthetic inference logs with progressively increasing noise, designed to test the full adaptation loop: diagnosis, curriculum synthesis, retraining, and verification. Across eight cold-start benchmarks spanning reasoning, math, code generation, summarization, and classification, Pioneer Agent improves over base models by 1.6-83.8 points. On AdaptFT-Bench, it improves or preserves performance in all seven scenarios, while naive retraining degrades by up to 43 points. On two production-style deployments built from public benchmark tasks, it raises intent classification from 84.9% to 99.3% and Entity F1 from 0.345 to 0.810. Beyond performance gains, the agent often discovers effective training strategies, including chain-of-thought supervision, task-specific optimization, and quality-focused data curation, purely from downstream feedback.

==> paper_figures/main_figure.tex <==
\resizebox{\textwidth}{!}{%
\begin{tikzpicture}[
    >=Stealth,
    node distance=0.9cm and 1.2cm,
    box/.style={
      rectangle, rounded corners=4pt, draw=black!70, thick,
      fill=white, minimum width=3.2cm, minimum height=0.9cm,
      text width=3cm, align=center, font=\small
    },
    decision/.style={
      diamond, draw=black!70, thick, fill=white,
      minimum width=1.4cm, minimum height=1.4cm,
      inner sep=1pt, align=center, font=\small
    },
    stackbox/.style={
      rectangle, rounded corners=4pt, draw=orange!60!black!40, thick,
      fill=orange!15, minimum width=4.8cm, minimum height=0.95cm,
      text width=4.6cm, align=center, font=\small
    },
    arr/.style={->, thick, black!70},
    redarr/.style={->, thick, red!70!black},
    greenarr/.style={->, thick, green!50!black},
    treenode/.style={circle, fill=black, inner sep=0pt, minimum size=5pt},
    treered/.style={circle, fill=red!70!black, inner sep=0pt, minimum size=5pt},
    treegreen/.style={circle, fill=green!50!black, inner sep=0pt, minimum size=5pt},
  ]

  % ===== COLUMN HEADERS =====
  \node[font=\bfseries\small] (coldlabel) at (0, 0) {COLD-START};
  \node[font=\bfseries\small] (prodlabel) at (5, 0) {PRODUCTION};

  % ===== COLD-START COLUMN =====
  \node[box, below=0.4cm of coldlabel] (cs1) {``Fine-tune Llama 3B\\on ARC''};
  \node[box, below=0.45cm of cs1] (cs2) {Research};

  \draw[arr] (cs1) -- (cs2);

  % ===== PRODUCTION COLUMN =====
  \node[box, below=0.4cm of prodlabel] (pr1) {Deployed model +\\production logs};
  \node[box, below=0.45cm of pr1] (pr2) {Diagnose and cluster\\deficiencies};
  \node[box, below=0.45cm of pr2] (pr3) {Synthesize\\Curriculum};

  \draw[arr] (pr1) -- (pr2);
  \draw[arr] (pr2) -- (pr3);

  % Align Curate data to same vertical position as Synthesize Curriculum
  \node[box] (cs3) at (cs2 |- pr3) {Curate data};
  \draw[arr] (cs2) -- (cs3);

  % ===== MCGS BOX =====
  \coordinate (mcgsTop) at ($(cs3.south)!0.5!(pr3.south) + (0, -0.9)$);

  % Tree nodes (left side of MCGS box)
  \node[treenode] (t1) at ($(mcgsTop) + (-3.2, -0.5)$) {};
  \node[treenode] (t2) at ($(t1) + (-0.7, -0.65)$) {};
  \node[treenode] (t3) at ($(t1) + (0.7, -0.65)$) {};
  \node[treered]   (t4) at ($(t2) + (-0.5, -0.65)$) {};
  \node[treegreen] (t5) at ($(t2) + (0.5, -0.65)$) {};
  \node[treenode]  (t6) at ($(t3) + (-0.5, -0.65)$) {};
  \node[treered]   (t7) at ($(t3) + (0.5, -0.65)$) {};
  \node[treegreen] (t8) at ($(t6) + (-0.4, -0.65)$) {};
  \node[treenode]  (t9) at ($(t6) + (0.4, -0.65)$) {};

  \draw[thick, black!70] (t1) -- (t2);
  \draw[thick, black!70] (t1) -- (t3);
  \draw[thick, black!70] (t2) -- (t4);
  \draw[thick, black!70] (t2) -- (t5);
  \draw[thick, black!70] (t3) -- (t6);
  \draw[thick, black!70] (t3) -- (t7);
  \draw[thick, black!70] (t6) -- (t8);
  \draw[thick, black!70] (t6) -- (t9);

  % MCGS title (two lines)
  \node[font=\bfseries\small, anchor=west, text width=4.5cm] (mcgsTitle)
    at ($(mcgsTop) + (-1.5, -0.35)$)
    {MCGS: Search Over\\Training Pipelines};

  % MCGS description text
  \node[anchor=north west, font=\ttfamily\scriptsize, inner sep=0pt, text width=5.5cm] (mcgsText)
    at ($(mcgsTitle.south west) + (0, -0.2)$)
    {Each Node $\pi$ = (Data, Config, Strategy)\\
     Expand: Reason about failures\\and explore\\
     Score: Eval\\
     Fuse: Combine winning branches\\
     Prune: Rollback any regress};

  % Draw the MCGS bounding box on the background layer
  \begin{scope}[on background layer]
    \node[rectangle, rounded corners=6pt, draw=black!70, thick,
          fill=white, fit=(t1)(t4)(t5)(t7)(t8)(t9)(mcgsTitle)(mcgsText),
          inner xsep=12pt, inner ysep=10pt] (mcgsBox) {};
  \end{scope}

  % Arrows from columns into MCGS box
  \draw[arr] (cs3.south) -- (cs3.south |- mcgsBox.north);
  \draw[arr] (pr3.south) -- (pr3.south |- mcgsBox.north);

  % ===== BOTTOM EVALUATION PIPELINE =====
  \node[box, minimum width=3cm, text width=2.8cm,
        below=1.8cm of mcgsBox.south west, anchor=north, xshift=0.3cm] (eval)
    {Evaluate on\\held out set};

  \node[decision, right=0.9cm of eval] (better) {Better?};

  \node[box, right=0.9cm of better, minimum width=2.6cm, text width=2.4cm] (reports) {Create Reports};

  \node[box, right=0.7cm of reports, minimum width=2cm, text width=1.8cm] (deploy) {Deploy};

  % Arrow from MCGS straight down, then left to Evaluate
  \draw[arr] (mcgsBox.south) -- ++(0,-0.5) -| (eval.north);

  % Evaluate -> Better
  \draw[arr] (eval) -- (better);

  % Better -> Create Reports (green)
  \draw[greenarr] (better) -- (reports);

  % Create Reports -> Deploy
  \draw[arr] (reports) -- (deploy);

  % Red feedback arrow: Better? straight up to MCGS box
  \draw[redarr] (better.north) -- (better.north |- mcgsBox.south);

  % Deploy -> Diagnose and cluster deficiencies
  \draw[arr, rounded corners=6pt] (deploy.north) -- (deploy.north |- pr2.east) -- (pr2.east);

  % ===== RIGHT SIDE: AGENT STACK (column 3) =====
  % Adjust this single value to control gap between boxes:
  \def\stackgap{0.65cm}

  \coordinate (stackAnchor) at (11.25, 0.3);

  \node[stackbox, anchor=north] (s1) at (stackAnchor) {%
    \textbf{Claude Sonnet 4.6}\\[-1pt]
    {\ttfamily\scriptsize 1M context, 32K thinking budget}};
  \node[stackbox, below=\stackgap of s1] (s2) {%
    \textbf{Tinker SDK}\\[-1pt]
    {\ttfamily\scriptsize LoRA fine-tuning, inference}};
  \node[stackbox, below=\stackgap of s2] (s3) {%
    \textbf{Sub-Agents}\\[-1pt]
    {\ttfamily\scriptsize Trace Analyzer, Task Delegation,\\[-2pt] shared /tmp/ filesystem}};
  \node[stackbox, below=\stackgap of s3] (s4) {%
    \textbf{Tools}\\[-1pt]
    {\ttfamily\scriptsize query\_traces, bash, web\_search,\\[-2pt] read/edit file, helper functions}};
  \node[stackbox, below=\stackgap of s4] (s5) {%
    \textbf{Context Manager}\\[-1pt]
    {\ttfamily\scriptsize Sustains 1000 turns}};
  \node[stackbox, below=\stackgap of s5] (s6) {%
    \textbf{Sandbox}\\[-1pt]
    {\ttfamily\scriptsize Modal, 16GB, 24h timeout,\\[-2pt] pre-injected data and helper functions}};
  \node[stackbox, below=\stackgap of s6] (s7) {%
    \textbf{External LLM APIs}\\[-1pt]
    {\ttfamily\scriptsize OpenAI, Deepseek, Fireworks\\[-2pt] Oracle distillation and LLM as judge}};

  % Outer container
  \coordinate (stackBot) at (stackAnchor |- deploy.south);
  \begin{scope}[on background layer]
    \node[rectangle, rounded corners=8pt, draw=orange!70!black, thick,
          fill=orange!8, fit=(s1)(s7)(stackBot),
          inner xsep=5pt, inner ysep=8pt] (stackOuter) {};
  \end{scope}

\end{tikzpicture}%
}

